Trust the Ray, Not the Depth: Ray-Lateral Agreement for Multi-View 3D Human Pose Fusion

Put a monocular mesh estimator behind every camera of a calibrated rig, and the reconstructed bodies land a meter or more apart. The cause is geometric: each estimate sits at the depth implied by a focal length the network assumed, not the one the camera has. Its error therefore points almost entirely along its own viewing ray, and the calibration tells us that direction exactly. To address this, we introduce the Ray-Lateral Agreement (RLA), which follows one rule: trust the ray, not the depth. RLA first slides every estimate along its own rays, which removes the depth bias and leaves the shape untouched. It then fuses the views one point at a time, under a Gaussian error whose precision follows each viewing ray. The maximum-likelihood solution is closed-form, interpolates between averaging and midpoint triangulation, and stays well conditioned where triangulation is singular. Robustness is the harder half, because correct views also disagree along their rays. Any weight built on the full residual therefore punishes good views together with bad ones. Ray-lateral agreement instead scores every view, at every point, by its residual across that view's own ray alone. We evaluated RLA on multi-camera public benchmark datasets. Across two, three, and four cameras and three per-view pose estimators, RLA consistently achieves lower worst-case error than all triangulation baselines.

==> supp_labels.tex <==
% Numbers of the supplementary material's sections, figures and tables cited in the main text;
% the supplement is not part of this version.
\makeatletter
\newlabel{fig:camera_count}{{6}{3}{\textbf {Error against camera count} on Panoptic: median (left) and 95th percentile (right, log scale) of MPJPE over camera subsets. All pairs; \pinfo {3}{subsets} random subsets with three and four cameras, \pinfo {5}{subsets} at each larger count marked, up to 25; and all 31 cameras together. We plot the 95th percentile because the maximum depends on how many subsets we sample. \method and the hybrid use held-out parameters}{figure.caption.35}{}}
\newlabel{fig:camera_count@cref}{{[figure][6][]6}{[1][2][]3}{}{}{}}
\newlabel{fig:supp_cameras}{{8}{4}{The 31 HD cameras of \texttt {171204\_pose1} seen from above, numbered as in the dataset; each triangle points along the camera's optical axis and is coloured by its height above the floor. Grey: the reference pelvis positions of the six people}{figure.caption.39}{}}
\newlabel{fig:supp_cameras@cref}{{[figure][8][]8}{[1][2][]4}{}{}{}}
\newlabel{fig:supp_failures}{{10}{6}{\textbf {Failures of \method } on Panoptic, chosen by rule as in \cref {fig:qualitative}: (g) its largest error over all pairs; (h) the pair and frame where its error exceeds that of DLT the most; (i) its largest error over all three-camera subsets}{figure.caption.43}{}}
\newlabel{fig:supp_failures@cref}{{[figure][10][]10}{[1][4][]6}{}{}{}}
\newlabel{fig:supp_qualitative}{{9}{5}{\textbf {More cases on Panoptic}, chosen by rule as in \cref {fig:qualitative}: (d) the largest error of DLT over all pairs; (e) that of RANSAC over all three-camera subsets; (f) a typical case, the median frame of the three-camera subset with the median error of \method }{figure.caption.42}{}}
\newlabel{fig:supp_qualitative@cref}{{[figure][9][]9}{[1][4][]5}{}{}{}}
\newlabel{fig:supp_subjects}{{7}{3}{The six people of Panoptic \texttt {171204\_pose1}, one frame each from camera 00\_05, with faces blurred}{figure.caption.37}{}}
\newlabel{fig:supp_subjects@cref}{{[figure][7][]7}{[1][2][]3}{}{}{}}
\newlabel{sec:exp_runtime}{{6.8}{6}{\texorpdfstring {\hskip -1em.~}{}Runtime}{subsection.6.8}{}}
\newlabel{sec:exp_runtime@cref}{{[subsection][8][6]6.8}{[1][6][]6}{}{}{}}
\newlabel{sec:supp_baselines}{{6.4}{1}{\texorpdfstring {\hskip -1em.~}{}Baselines}{subsection.6.4}{}}
\newlabel{sec:supp_baselines@cref}{{[subsection][4][6]6.4}{[1][1][]1}{}{}{}}
\newlabel{sec:supp_fit3d}{{6.10}{7}{\texorpdfstring {\hskip -1em.~}{}A second dataset: Fit3D}{subsection.6.10}{}}
\newlabel{sec:supp_fit3d@cref}{{[subsection][10][6]6.10}{[1][7][]7}{}{}{}}
\newlabel{sec:supp_hmr2}{{6.7}{4}{\texorpdfstring {\hskip -1em.~}{}Other per-view estimators}{subsection.6.7}{}}
\newlabel{sec:supp_hmr2@cref}{{[subsection][7][6]6.7}{[1][4][]4}{}{}{}}
\newlabel{sec:supp_mle}{{6.2}{1}{\texorpdfstring {\hskip -1em.~}{}Fusion as maximum likelihood}{subsection.6.2}{}}
\newlabel{sec:supp_mle@cref}{{[subsection][2][6]6.2}{[1][1][]1}{}{}{}}
\newlabel{sec:supp_panoptic}{{6.5}{2}{\texorpdfstring {\hskip -1em.~}{}Panoptic details}{subsection.6.5}{}}
\newlabel{sec:supp_panoptic@cref}{{[subsection][5][6]6.5}{[1][2][]2}{}{}{}}
\newlabel{sec:supp_qualitative}{{6.6}{2}{\texorpdfstring {\hskip -1em.~}{}Qualitative results}{subsection.6.6}{}}
\newlabel{sec:supp_qualitative@cref}{{[subsection][6][6]6.6}{[1][2][]2}{}{}{}}
\newlabel{sec:supp_seq2}{{6.9}{7}{\texorpdfstring {\hskip -1em.~}{}A second Panoptic sequence}{subsection.6.9}{}}
\newlabel{sec:supp_seq2@cref}{{[subsection][9][6]6.9}{[1][6][]7}{}{}{}}
\newlabel{sec:supp_shift}{{6.3}{1}{\texorpdfstring {\hskip -1em.~}{}Translating rather than rescaling the depth}{subsection.6.3}{}}
\newlabel{sec:supp_shift@cref}{{[subsection][3][6]6.3}{[1][1][]1}{}{}{}}
\newlabel{tab:ablation}{{2}{2}{\textbf {Ablation} on Panoptic: median over the \gnum {ab}{3@subsets} three-camera subsets of \cref {tab:panoptic} and the \gnum {ab}{5@subsets} five-camera subsets of \cref {fig:camera_count} (mm). Each fusion variant has its own parameters chosen by leave-one-subject-out from the grid used for \method . Bold: lowest per column}{table.caption.28}{}}
\newlabel{tab:ablation@cref}{{[table][2][]2}{[1][1][]2}{}{}{}}
\newlabel{tab:depth}{{4}{3}{\textbf {Depth correction} on Panoptic: median over the 31 single cameras and the \gnum {dc}{pairs} camera pairs; 507 frames, six subjects weighted equally (mm). Without correction, averaging misplaces the body by about a metre. Rescaling every depth compresses the body along the ray; translating along the ray (\cref {eq:shift}) keeps its shape. True $\mK _c$: SAM~3D~Body receives each camera's true intrinsics and needs no correction. Triangulation does not use the corrected depth. \method with the held-out parameters of \cref {tab:panoptic}}{table.caption.36}{}}
\newlabel{tab:depth@cref}{{[table][4][]4}{[1][2][]3}{}{}{}}
\newlabel{tab:hmr2}{{8}{7}{\textbf {Other per-view estimators} on the camera subsets of \cref {tab:panoptic}: median and worst MPJPE over subsets (mm). CameraHMR with its own focal-length estimate, corrected by \cref {eq:shift}. RANSAC at the 20\,px of \cref {tab:panoptic}, and with its threshold $\tau $ chosen by leave-one-subject-out (three or more cameras); hybrid: RANSAC set (20\,px) + \method ; held-out parameters. PA-MPJPE and all baselines: \cref {tab:supp_hmr2,tab:supp_camerahmr_fov}. Bold: best per column and estimator}{table.caption.44}{}}
\newlabel{tab:hmr2@cref}{{[table][8][]8}{[1][5][]7}{}{}{}}
\newlabel{tab:supp_bones}{{5}{3}{Median reference bone lengths per identity of \texttt {171204\_pose1}. They differ by up to \gnum {bl}{spread}\%, consistent with six different people rather than re-tracks of one}{table.caption.38}{}}
\newlabel{tab:supp_bones@cref}{{[table][5][]5}{[1][2][]3}{}{}{}}
\newlabel{tab:supp_camerahmr}{{11}{9}{\textbf {CameraHMR given each camera's true focal length}: the camera subsets, frames and methods of \cref {tab:panoptic} (mm). Held-out: $(\lambda ,\alpha )$ chosen by leave-one-subject-out. Bold: best in each column}{table.caption.50}{}}
\newlabel{tab:supp_camerahmr@cref}{{[table][11][]11}{[1][6][]9}{}{}{}}
\newlabel{tab:supp_camerahmr_fov}{{10}{8}{\textbf {CameraHMR as the per-view estimator}, with its own focal-length estimate (HumanFoV) corrected by \cref {eq:shift}: the camera subsets, frames and methods of \cref {tab:panoptic} (mm). Held-out: $(\lambda ,\alpha )$ chosen by leave-one-subject-out. Bold: best in each column}{table.caption.49}{}}
\newlabel{tab:supp_camerahmr_fov@cref}{{[table][10][]10}{[1][6][]8}{}{}{}}
\newlabel{tab:supp_detector}{{3}{3}{\textbf {The 2D detector pipeline} on the camera subsets of \cref {tab:panoptic}: YOLOv8x-pose keypoints triangulated four ways, scored on the joints each method produces (coverage: the share of the $507\times 17$ joints with a result, mean over subsets); the SAM~3D~Body rows are from \cref {tab:panoptic}, with held-out parameters, and cover every joint. Median and worst over subsets, six subjects weighted equally (mm). Bold: best in each column}{table.caption.33}{}}
\newlabel{tab:supp_detector@cref}{{[table][3][]3}{[1][2][]3}{}{}{}}
\newlabel{tab:supp_hmr2}{{9}{8}{\textbf {HMR~2.0 as the per-view estimator}: the camera subsets, frames and methods of \cref {tab:panoptic} (mm). Held-out: $(\lambda ,\alpha )$ chosen by leave-one-subject-out. Bold: best in each column}{table.caption.48}{}}
\newlabel{tab:supp_hmr2@cref}{{[table][9][]9}{[1][6][]8}{}{}{}}
\newlabel{tab:supp_joints}{{7}{4}{\textbf {Per joint} on Panoptic: median MPJPE over the \gnum {sj}{subsets} four-camera subsets of \cref {tab:panoptic}, left and right joints averaged, subjects weighted equally (mm). Parameters as in \cref {tab:supp_subjects}. Bold: lowest per joint}{table.caption.41}{}}
\newlabel{tab:supp_joints@cref}{{[table][7][]7}{[1][2][]4}{}{}{}}
\newlabel{tab:supp_seq2}{{12}{9}{\textbf {A second Panoptic sequence} (\texttt {\gnum {p2}{name}}, \gnum {p2}{subjects} subjects weighted equally, \gnum {p2}{scored} frames): every pair, and random subsets of three and four of the 31 HD cameras (mm). The setting of $(\lambda ,\alpha )$ per camera count is the one selected on the first sequence; nothing is tuned here. Bold: best in each column}{table.caption.51}{}}
\newlabel{tab:supp_seq2@cref}{{[table][12][]12}{[1][6][]9}{}{}{}}
\newlabel{tab:supp_subjects}{{6}{4}{\textbf {Per subject} on Panoptic: for each subject, the median MPJPE over the subsets of \cref {tab:panoptic} (mm). \method and the hybrid use the setting chosen on the other five subjects; All: the median of the six-subject mean, as in \cref {tab:panoptic}. With two cameras, DLT+IRLS and RANSAC reduce to DLT. Bold: lowest per subject and camera count}{table.caption.40}{}}
\newlabel{tab:supp_subjects@cref}{{[table][6][]6}{[1][2][]4}{}{}{}}
\makeatother

